Practical Efficiency of Muon for Pretraining

We demonstrate that Muon, the simplest instantiation of a second-order optimizer, explicitly expands the Pareto frontier over AdamW on the compute-time tradeoff. We find that Muon is more effective than AdamW in retaining data efficiency at large batch sizes, far beyond the so-called critical batch size, while remaining computationally efficient, thus enabling more economical training. We study the combination of Muon and the maximal update parameterization (muP) for efficient hyperparameter transfer and present a simple telescoping algorithm that accounts for all sources of error in muP while introducing only a modest overhead in resources. We validate our findings through extensive experiments with model sizes up to four billion parameters and ablations on the data distribution and architecture.

==> critical_batch_size.tex <==
\subsection{Formalizing the Critical Batch Size}
\label{app:formal-critical}

To get a sense of the work involved in formalizing the critical batch size, consider the framework of  \citet{mccandlish2018empirical} who study the expected one-step loss under optimal SGD with batch size $B$ and show that 
\begin{align*}
    \min_{\eta \in \R}\; \expect{L\paren{\theta - \eta \frac{\sum_{i=1}^B \nabla L_{x_i}(\theta)}{B}}} \approx L(\theta) - \frac{\Delta L_{\max}(\theta)}{1 + B_{\mathrm{noise}}(\theta)/B}
\end{align*}
where the approximation comes from a second-order Taylor expansion. 
The term $B_{\mathrm{noise}}(\theta)/B$ can be viewed as a noise-to-signal ratio (NSR) for the gradient estimate. 
As $B$ grows, the loss reduction approaches the ceiling $\Delta L_{\max}(\theta)$, but the marginal gain begins to diminish once $B$ is on the order of the ``gradient noise scale'' $B_{\mathrm{noise}}(\theta)$.

While $B_{\mathrm{noise}}(\theta)$ is well defined (a function of the gradient and the Hessian), it is difficult to estimate in practice and motivates a series of further simplifications. In the end, the authors define the critical batch size as the ratio of the theoretically minimum number of examples and steps to reach a target loss $B_{\mathrm{crit}}(L^\star)=E_{\min}/S_{\min}$, estimate $E_{\min}$ and $S_{\min}$ from an empirical fit to a certain formula, and justify it as a weighted average of the gradient noise scale along the optimization path. 

==> formal_slope.tex <==
\subsection{Proof that the Critical Batch Size Slope is $-1$}
\label{app:formal-slope}

Let $S$ denote the number of steps to reach some target loss. The piecewise linear assumption between $S$ and the batch size $B$ in log-log scale is
\begin{align}
    \log S = m \log B + b  \label{eq:loglinear}
\end{align}
for some locally constant slope $m$ and intercept $b$. The batch size $B$ is in the perfect scaling regime (i.e., does not exceed the critical batch size) if the total number of training tokens $T$ required to reach the loss does not change in $B$.
Since $T = BS$ and $S = 2^b B^m$ from \eqref{eq:loglinear}, we have 
\begin{align}
    T = 2^b B^{m+1} \label{eq:loglinear2}
\end{align}
Thus we have a constant $T = 2^b$ iff $m = -1$. 
For $m \neq -1$, we have an exponential relationship $T = O(B^{m+1})$  (decreasing if $m < -1$, increasing if $m > -1$).

==> karl_scratch.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\hspace{-4mm}\includegraphics[width=7cm]{karl_images/1b_token_ratio.pdf}
& 
\hspace{-2mm}\includegraphics[width=7cm]{karl_images/1b_token_advantage.pdf}
\end{tabular}
\end{center}
\caption{(Left) Token ratio vs batch size plots for different target losses. (Right) Token difference increases in batch size.}
\label{fig:token-ratio}
\end{figure}


\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\hspace{-3mm}\includegraphics[width=6.9cm]{karl_images/tradeoff.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/tradeoff_py_1.3.pdf}\\
\hspace{-3mm}\includegraphics[width=6.9cm]{karl_images/tradeoff_py_1.8.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/tradeoff_dclm_3.25.pdf}
\end{tabular}
\end{center}
\caption{(Top left) Illustration of the compute-time tradeoff. Optimizers are represented as iso-loss curves on the compute-time plane. Economically feasible training options are shaded in blue. New options (e.g., shorter run, fewer devices) enabled by Optimizer 2 are shaded in green. (Others) Empirical observations.}
\label{fig:tradeoff-main}
\end{figure}

The empirical fact that $R_L(B) = \frac{T_{L,A}(B)}{T_{L,M}(B)} > 1$ is nondecreasing (often increasing) means the non-optimizer FLOP overhead $F_A(B) - F_M(B)$ of AdamW is a constant (or growing) percentage of Muon's FLOPs $F_M(B)$ even for large values of $B$. At the same time, for a sufficiently large $B$, the FLOP overhead of Muon over Adam diminishes as $\Theta(\frac{1}{B})$, making the total FLOPs/second for both optimizers roughly similar to $\wb{F}$. Then the ratio between the training time under AdamW $\frac{F_A(B)}{\wb{F}}$ and Muon $\frac{F_M(B)}{\wb{F}}$ is approximately $R_L(B) > 1$.


If we assume $B_{L,A}^\star < B_{L,M}^\star$ (i.e., AdamW has a smaller critical batch size compared to Muon), we have 
$R_L(B) = T_{L,A}^\star/ T_{L,M}^\star$ for $B \leq B_{L, A}^\star$, 
$R_L(B) = \mathrm{inc}_A(B) / T_{L,M}^\star$ for $B_{L, A}^\star < B \leq B_{L, M}^\star$, and 
$R_L(B) = \mathrm{inc}_A(B) / \mathrm{inc}_M(B)$ for $B > B_{L, M}^\star$.
See Figure~\ref{fig:token-ratio} left for an illustration.


\begin{align}
    \frac{\partial \log A(L, B) }{\partial \log B} = \begin{cases} 0 &\text{for $B \leq B_{\mathrm{crit}, A}(L)$} \\ 
    m_A + 1 &\text{for $B_{\mathrm{crit}, A}(L) < B \leq B_{\mathrm{crit}, M}(L)$} \\
    m_A - m_M &\text{for $B > B_{\mathrm{crit}, M}(L)$}
    \end{cases} \label{eq:adv-slope}
\end{align}


Despite the simple intuition, formalizing the critical batch size can be nontrivial (Appendix~\ref{app:formal-critical}). 
An empirical approach is to measure the number of steps $S(L, B)$ required to reach a target loss $L$ as a function of the batch size $B$. 
Researchers have found that this plot often exhibits a roughly piecewise linear relationship between $S(L, B)$ and $B$ in log-log scale with a ``phase transition'' from perfect scaling to imperfect.
The critical batch size can then be formulated as a value $B_{\mathrm{crit}}(L)$ such that 
\begin{align}
    \log S(L, B) = \begin{cases} - \log B + b_1 &\text{for $B \leq B_{\mathrm{crit}}(L)$} \\ m \log B + b_2 &\text{for $B > B_{\mathrm{crit}}(L)$, where $-1 < m < 0$} \end{cases} \label{eq:crit}
\end{align}
with some intercepts $b_1, b_2$ (Appendix~\ref{app:formal-slope}).
Thus an optimizer is argued as enjoying a larger critical batch size if the transition (i.e., kink) seems to happen at a larger batch size \citep{zhang2019algorithmic,vyas2024soap}.


\vspace{50mm}
Instead of using a point estimate such as the critical batch size or the token-optimal batch size, we propose to monitor how $A_{M,A}(L,B)$ changes in $B$ to fully characterize the data efficiency benefit of Muon over AdamW in batch sizes. In an idealized setting with unique values  $B_{\mathrm{crit}, A}(L)$ and $B_{\mathrm{crit}, M}(L)$ of the critical batch size for AdamW and Muon beyond which the rate of diminishing returns is the same, $A_{M,A}(L, B)$ should exhibit a piecewise linear relationship with $B$ as shown in Figure~\ref{fig:token-advantage} left where the token advantage eventually becomes constant.



\subsection{Existing Batch Size Research}
\label{sec:batch-size}

Increasing the batch size is one of the easiest ways to accelerate training on data parallel hardware.\footnote{To keep the discussion simple, we assume that the per-device batch size is large enough to saturate the device MFU. Thus adding devices corresponds to increasing the batch size in a straightforward manner.}
A great deal of research focuses on the idea of ``critical'' batch size, which is broadly defined as the largest batch size that allows for perfect scaling (i.e. doubling the batch size halves the number of steps) beyond which we receive diminishing returns \citep{balles2016coupling,goyal2017accurate,mccandlish2018empirical,zhang2019algorithmic,shallue2019measuring}. 


\vspace{-0mm}
\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\hspace{-1mm}\includegraphics[width=6.9cm]{karl_images/500m_batch_pydc_3p6.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/500m_batch_pydc_2p15.pdf}
\end{tabular}
\end{center}
\caption{Steps-to-loss vs batch size plots with 500M parameter models on the Python+DCLM mix (see Appendix~\ref{app:steps-loss} for plots on separate distributions). The right plot uses the lowest loss achieved by both AdamW and Muon as the target loss. While Muon requires fewer steps than AdamW at all batch sizes, it is not apparent how to pinpoint a single phase transition, particularly at a low target loss.}
\label{fig:steps-batch}
\end{figure}

Despite the simple intuition, formalizing the critical batch size is nontrivial and 
necessitates a host of assumptions that do not hold in practice 
(Appendix~\ref{app:formal-critical}). 
As a result, many researchers simply gauge the critical batch size from empirical data. One such approach is to plot the number of steps $S_o(L, B)$ under optimizer $o$ required to reach a target loss $L$ as a function of the batch size $B$. 
Researchers have found that this plot often exhibits a roughly log-linear relationship between $S_o(L, B)$ and $B$ with a ``phase transition'' from perfect scaling to imperfect.
Thus an optimizer is argued as enjoying a larger critical batch size if the transition seems to happen at a larger batch size \citep{zhang2019algorithmic,vyas2024soap}.

We plot the steps $S_A(L, B)$ for AdamW  and $S_M(L, B)$ Muon in Figure~\ref{fig:steps-batch}, using model size 500M on Python and DCLM data and varying batch sizes up to 16M.  
While we generally observe that $S_M(L, B) < S_A(L, B)$ for all $L$ and $B$, the plots are limiting for the purpose of critical batch size study for the following reasons. First, they do not always exhibit a clear phase transition (e.g., there may be no major kink, or there may be multiple), particularly at a low target loss. 
%Thus we find it limiting to  gauging the critical batch size from these plots. 
Second, the semantics of the plot is tightly coupled with the slope. If the slope is larger than $-1$, it implies that we should use a smaller batch size regardless of any kink since we are already in the regime of diminishing returns. Conversely, if the slope is smaller than $-1$, there can be several kinks but none of them is a critical batch size. See Appendix~\ref{app:formal-slope} for more detail. Thus without reporting the actual slope value, the visual presence of phrase transitions alone can be misleading. 

\vspace{-0mm}
\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\hspace{-1mm}\includegraphics[width=6.4cm]{karl_images/toy_figure.pdf}
& 
\hspace{-4mm}\includegraphics[width=7cm]{karl_images/toks2loss_1b_2p8.pdf}
\end{tabular}
\end{center}
\caption{(Left) Illustration of the tokens-to-loss vs batch size plot under an idealized setting with one critical batch size. (Right) Empirical observations.}
\label{fig:tok-opt}
\end{figure}

\subsection{Token-Optimal Batch Size}
\label{sec:token-efficiency}

As a first step toward a more effective measurement of optimal batch size, we propose a simple reparameterization of the steps-to-loss plot. Specifically, we scale the steps by batch sizes and plot the number of tokens $T_o(L, B) = B \times S_o(L, B)$ consumed by $o \in \myset{A, M}$ (Adam or Muon) to reach loss $L$ using batch size $B$. In an idealized setting with a unique value  $B_{\mathrm{crit}, o}(L)$ of the critical batch size, $T_o(L, B)$ should remain constant for all $B \leq B_{\mathrm{crit}}(L)$ and then  monotonically increase (Figure~\ref{fig:tok-opt}). We can then define a ``token-optimal'' batch size as the largest batch size that reaches the lowest point on this curve:
\begin{align}
    B_{\mathrm{tok}, o}(L) = \max \myset{B:\; T_o(L, B) = \min_{B'} T_o(L, B')} \label{eq:tok-opt}
\end{align}
In the idealized setting, $B_{\mathrm{tok},o}(L)$ coincides with the kink in the steps-to-loss plot. But unlike the kink, $B_{\mathrm{tok}}(L)$ is always uniquely defined and thus allows for convenient measurement. $B_{\mathrm{tok},o}(L)$ also has the clear semantics of being the most data-efficient batch size.

\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\hspace{-1mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_py_gemma3_adamw.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_py_gemma3_muon.pdf} 
\end{tabular}
\end{center}
\caption{Comparison of the change in the token-optimal batch size \eqref{eq:tok-opt} throughout training between AdamW and Muon. The black line displays the token-optimal batch size across different loss thresholds near convergence.}
\label{fig:token-eff-plots}
\end{figure}

We can obtain a more informative plot by inspecting $B_{\mathrm{tok},o}(L)$ across different values of $L$, corresponding to how the token-optimal batch size changes throughout training.
Figure~\ref{fig:token-eff-plots} plots $B_{\mathrm{tok},A}(L)$ and $B_{\mathrm{tok},M}(L)$ for various loss thresholds near convergence. We see that the token-optimal batch size increases during training, which is consistent with the predicted behavior of critical batch size \citep{mccandlish2018empirical}. 
We observe that $B_{\mathrm{tok},M}(L) \geq B_{\mathrm{tok},A}(L)$ in general (e.g., 2M vs 3.5M at convergence in these plots), suggesting that Muon allows for a larger token-optimal batch size over AdamW. We give ablations on the architecture, dataset, and model size in Appendix~\ref{app:tokens-loss}.

\subsubsection{Limitations}
While the token-optimal batch size gives us a well-defined notion of optimality (unlike the kinks in the steps-to-loss plot), it suffers from severe limitations.
First, the quantity is brittle under noise. It is easy to construct an example with $T_o(L, B) \approx T_{o'}(L, B)$ (i.e., nearly identical tokens-to-loss curves) in which a tiny perturbation flips $B_{tok,o}(L) \gg B_{tok,o'}(L)$ to $B_{tok,o}(L) \ll B_{tok,o'}(L)$. Second, much more seriously,  
the quantity is still a point estimate and fails to communicate the full batch size benefit of Muon over AdamW.
For instance, in Figure~\ref{fig:token-eff-plots}, $B_{tok,A}(1.35) = B_{tok,M}(1.35) = 2e6$ (i.e., AdamW and Muon have the same token-optimal batch size). However, $T_M(1.35, B)$ increases much more slowly than $T_A(1.35, B)$ as we increase $B > 2e6$. This over-large batch size behavior can play a critical role in the compute-time tradeoff. 

\subsection{Token Advantage}
\label{sec:token-advantage}

We define the ``token advantage'' of Muon over AdamW at batch size $B$ as how many additional tokens AdamW requires compared to Muon to reach the same target loss:
\begin{align}
    A_{M,A}(L, B) = T_A(L, B) - T_M(L, B) \label{eq:token-advantage}
\end{align}
Instead of using a point estimate such as the critical batch size or the token-optimal batch size, we propose to monitor how $A_{M,A}(L,B)$ changes in $B$ to fully characterize the data efficiency benefit of Muon over AdamW in batch sizes. In an idealized setting with unique values  $B_{\mathrm{crit}, A}(L)$ and $B_{\mathrm{crit}, M}(L)$ of the critical batch size for AdamW and Muon beyond which the rate of diminishing returns is the same, $A_{M,A}(L, B)$ should exhibit a piecewise linear relationship with $B$ as shown in Figure~\ref{fig:token-advantage} left where the token advantage eventually becomes constant.


\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\hspace{-4mm}\includegraphics[width=5.1cm]{karl_images/toy_figure2.pdf}
& 
\hspace{-2mm}\includegraphics[width=7.8cm]{karl_images/4b_token_advantage.pdf} 
\end{tabular}
\end{center}
\caption{(Left) Illustration of the token advantage vs batch size plot under an idealized setting with one critical batch size after which the rate of diminishing returns is the same. (Right) Empirical observations.}
\label{fig:token-advantage}
\end{figure}

\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\hspace{-3mm}\includegraphics[width=6.5cm]{karl_images/tok_adv_models_3.2.pdf}
& 
\hspace{-4mm}\includegraphics[width=7.3cm]{karl_images/4b_token_advantage_percentage.pdf} 
\end{tabular}
\end{center}
\caption{Test}
\label{fig:token-advantage-2}
\end{figure}

However, we empirically observe that the token advantage continues to increase beyond any particular batch sizes (Figure~\ref{fig:token-advantage} right).
Our finding suggests that Muon keeps improving the relative data efficiency over AdamW as we keep pushing the batch size larger---beyond any single point such as the critical or token-optimal batch size.



==> steps_loss_extra.tex <==


\subsection{Additional Steps-to-Loss vs Batch Size Plots}
\label{app:steps-loss}

Figure~\ref{fig:steps-batch-extra} shows the steps-to-loss vs batch size plots on Python and DCLM. The overall trend is the same as Python+DCLM (Figure~\ref{fig:steps-batch}), namely (1) Muon requires fewer steps at all batch sizes, (2) it is not clear how to identify critical batch sizes, especially at lower target losses.


\vspace{-0mm}
\begin{figure}[t!]
\begin{center}
\begin{tabular}{cc}
\hspace{-1mm}\includegraphics[width=6.5cm]{karl_images/500m_batch_py_2p4.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.5cm]{karl_images/500m_batch_py_1p3.pdf} \\
\hspace{-1mm}\includegraphics[width=6.5cm]{karl_images/500m_batch_dclm_4p0.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.5cm]{karl_images/500m_batch_dclm_3p1.pdf}
\end{tabular}
\end{center}
\caption{Steps-to-loss vs batch size plots (log-log scale) with 500M parameter models on Python and DCLM.}
\label{fig:steps-batch-extra}
\end{figure}

==> token_advantage_extra.tex <==
\subsection{Additional Token Ratio Plots}
\label{app:token-ratio}


Figure~\ref{fig:token-ratio-model-sizes} shows the token ratio plots for 2B and 4B model sizes. As in the 1B model size (Figure~\ref{fig:token-ratio}), we see that the token ratio between AdamW and Muon is above 1 and generally increasing or constant at all thresholds.

\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\hspace{-3mm}\includegraphics[width=7cm]{karl_images/2b_token_ratio.pdf}
& 
\hspace{-4mm}\includegraphics[width=7cm]{karl_images/4b_token_ratio.pdf}
\end{tabular} 
\end{center}
\caption{Token ratio plots for 2B and 4B model sizes (see Figure~\ref{fig:tok-opt} for 1B)}
\label{fig:token-ratio-model-sizes}
\end{figure}


Figure~\ref{fig:token-diff-model-sizes-fixed} plots the additional number of tokens required by AdamW at fixed target thresholds on DCLM across 1B, 2B, and 4B. We see that the extra number of tokens increases in the batch size and is furthermore largely agnostic to the model size at all thresholds.


\begin{figure}[t]
\begin{center}
\begin{tabular}{cc}
\hspace{-3mm}\includegraphics[width=7cm]{karl_images/tok_adv_models_2.8.pdf}
& 
\hspace{-4mm}\includegraphics[width=7cm]{karl_images/tok_adv_models_3.2.pdf} \\
\hspace{-3mm}\includegraphics[width=7cm]{karl_images/tok_adv_models_3.6.pdf}
& 
\hspace{-4mm}\includegraphics[width=7cm]{karl_images/tok_adv_models_4.0.pdf} 
\end{tabular} 
\end{center}
\caption{Number of additional tokens required by AdamW over Muon at different loss thresholds  across model sizes (DCLM)}
\label{fig:token-diff-model-sizes-fixed}
\end{figure}


==> tokens_loss_extra.tex <==
\subsection{Additional Tokens-to-Loss vs Batch Size Plots}
\label{app:tokens-loss}

\paragraph{Architecture ablation.}  Figure~\ref{fig:token-eff-plots-arch} shows the token-optimal batch size plots using Gemma 2 as the architecture instead of Gemma 3 (i.e., QK-norm instead of soft-capping) on Python. Muon increases the token-optimal batch sizes over AdamW at all thresholds.

\begin{figure}[t!]
\begin{center}
\begin{tabular}{cc}
\hspace{-1mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_py_gemma3_adamw.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_py_gemma3_muon.pdf}\\
\hspace{-1mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_py_gemma2_adamw.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_py_gemma2_muon.pdf}
\end{tabular}
\end{center}
\caption{Token-optimal batch size plots: architecture ablation (Gemma 3 vs Gemma 2)}
\label{fig:token-eff-plots-arch}
\end{figure}


\paragraph{Dataset ablation.} Figure~\ref{fig:token-eff-plots-data} shows the token-optimal batch size plots on Python+DCLM and DCLM.
Muon generally increases the token-optimal batch sizes over AdamW on these datasets. While the difference is less pronounced as we move from Python to DCLM, Muon increases much more gradually in the number of tokens beyond the token-optimal batch size compared to AdamW.



\begin{figure}[t!]
\begin{center}
\begin{tabular}{cc}
\hspace{-1mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_pydc_gemma3_adamw.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_pydc_gemma3_muon.pdf} \\
\hspace{-1mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_dclm_gemma3_2_adamw.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_500m_dclm_gemma3_muon.pdf}
\end{tabular}
\end{center}
\caption{Token-optimal batch size plots: dataset ablation (Python+DCLM and DCLM)}
\label{fig:token-eff-plots-data}
\end{figure}


\paragraph{Model size ablation.} Figure~\ref{fig:token-eff-plots-model-size} shows the token-optimal batch size  plots on 1B, 2B, and 4B parameter models on DCLM.
Muon generally has a larger token-optimal batch size than AdamW across the model sizes.


\begin{figure}[ht!]
\begin{center}
\begin{tabular}{cc}
\hspace{-1mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_1b_dclm_gemma3_adamw.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_1b_dclm_gemma3_muon.pdf} \\
\hspace{-1mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_2b_dclm_gemma3_adamw.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_2b_dclm_gemma3_muon.pdf} \\
\hspace{-1mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_4b_dclm_gemma3_adamw.pdf}
& 
\hspace{-4mm}\includegraphics[width=6.9cm]{karl_images/combined_thresholds_4b_dclm_gemma3_muon.pdf} 
\end{tabular}
\end{center}
\caption{Token-optimal batch size plots: model size ablation (1B, 2B, and 4B)}
\label{fig:token-eff-plots-model-size}
\end{figure}

